Black Box Adversarial Prompting for Foundation Models

Prompting interfaces allow users to quickly adjust the output of generative models in both vision and language. However, small changes and design choices in the prompt can lead to significant differences in the output. In this work, we develop a black-box framework for generating adversarial prompts for unstructured image and text generation. These prompts, which can be standalone or prepended to benign prompts, induce specific behaviors into the generative process, such as generating images of a particular object or generating high perplexity text.

==> icml_workshop/experiments_workshop.tex <==

Utilizing the Token Space Projection discussed in \Cref{sec: token space projection}, we apply the two black-box optimization methods discussed in \Cref{sec: opt approaches} to each task introduced in \Cref{sec: threat models}. For the text-to-image tasks, we use embeddings from CLIP ViT-L/14 tokenizer \citep{Radford2021LearningTV} where $m=768$, and optimize over $d=4$ tokens. For the text-to-text tasks, we use embeddings from the L-2 H-128 BERT model \citep{Turc2019WellReadSL} where $m=128$, and optimize  over $d=6$ tokens.
Code to reproduce all results is available at \url{https://blinded-url}. Implementation details and hyperparameters are detailed in Appendix~\ref{app:implementation}. 
\subsection{Image Generation}
We consider the optimization Tasks \ref{task: unrestricted prompts 1}, \ref{task: restricted prompts 2}, and \ref{task: restricted prepending prompts 3} as described in \Cref{sec: loss and threats} using the Classifier Loss. We use the Stable Diffusion v1.5 model \citep{StableDiff} to generate 512x512 images, using a classifier free guidance scale of 7.5 \citep{ho2021classifierfree} and 25 inference steps with the default scheduler. For our classifier loss function, we use the standard ResNet18 from TorchVision \citep{torchvision2016} and use the negative log class probability for the desired class.

For Tasks \ref{task: unrestricted prompts 1} and \ref{task: restricted prompts 2}, we allow the black-box optimization methods to query a total of 5,000 prompts before terminating. If the optimizer fails to make progress for 1,000 prompt consecutive queries, we terminate early. Since Task \ref{task: restricted prepending prompts 3} is more difficult, we allow 10,000 prompts to be queried and terminate early after failing to make progress for 3,000 consecutive queries.

\subsubsection{Quantitative Evaluation Metrics}
\label{sec:success-methods}
\input{results_table.tex}
In addition to example images demonstrating success, we measure the \textit{success} of optimized prompts quantitatively in two ways.
\vspace{-2ex}
\paragraph{Most Probable Class Success (MPC Success).} The optimizer achieves \textit{MPC success} if it finds a prompt for which the target class is the largest probability class for the majority of 5 images generated according to a pretrained ResNet18 classification model.
\vspace{-2ex}
\paragraph{Out-Performing Simple Baseline Prompts (OPB Success).} Denote by \CLS{} the target ImageNet class. We compute the loss using the following two baseline prompts: \CLS{} and \texttt{a picture of a \CLS{}}. The optimizer achieves \textit{OPB success} if the optimizer finds a prompt that achieves lower loss than both of these baseline prompts.

\begin{figure}[t]
\centering
% \begin{subfigure}[b]{0.48\textwidth}
% %\centering
% \addtolength{\tabcolsep}{-5.5pt}   
% \begin{tabular}{lll}
% \multicolumn{3}{l} {\fontsize{11pt}{13pt}\textbf{Goal Class:} \texttt{lizard}}\\
%      \multicolumn{3}{l} {\ttbfs{louisiana argonhilton deta}}\\
%      \includegraphics[width=0.333\columnwidth]{final_images/lizard/louisiana_argonhilton_deta.jpg} &
%      \includegraphics[width=0.333\columnwidth]{final_images/lizard/louisiana_argonhilton_deta_1.jpg} &
%      \includegraphics[width=0.333\columnwidth]{final_images/lizard/louisiana_argonhilton_deta_2.jpg}
% \end{tabular}
% \newline
% \begin{tabular}{llll}
%     \ttbfs{louisiana} & \ttbfs{argon} & \ttbfs{hilton} & \ttbfs{deta} \\
%     \includegraphics[width=0.25\columnwidth]{final_images/lizard/louisiana_3.jpg} &
%     \includegraphics[width=0.25\columnwidth]{final_images/lizard/argon_2.jpg} &
%     \includegraphics[width=0.25\columnwidth]{final_images/lizard/hilton.jpg} & 
%     \includegraphics[width=0.25\columnwidth]{final_images/lizard/deta.jpg}
% \end{tabular}

% \caption{Task \ref{task: restricted prompts 2} generated images with the class \texttt{lizard}.}
% \label{lizard-and-lipstick}
% \end{subfigure}
%\hfill
%\begin{subfigure}[b]{0.48\textwidth}
\centering
\addtolength{\tabcolsep}{-5.5pt}   
\begin{tabular}{lll}
    \multicolumn{3}{l} {\fontsize{11pt}{13pt}\textbf{Goal Class:} \texttt{aircraft}}\\
     \multicolumn{3}{l} {{\fontsize{8pt}{10pt}\ttbfs{pegasus yorkshire wwii taken a picture of the ocean}} {} }\\
     \includegraphics[width=0.333\columnwidth]{final_images/aircraft/pegasus_yorkshire_wwii_taken_a_picture_of_the_ocean.jpg} &
     \includegraphics[width=0.333\columnwidth]{final_images/aircraft/pegasus_yorkshire_wwii_taken_a_picture_of_the_ocean_1.jpg} &
     \includegraphics[width=0.333\columnwidth]{final_images/aircraft/pegasus_yorkshire_wwii_taken_a_picture_of_the_ocean_2.jpg}
\end{tabular}
\newline
\begin{tabular}{llll}
    \ttbfs{pegasus} & \ttbfs{yorkshire} & \ttbfs{wwii} & \ttbfs{taken} \\
    \includegraphics[width=0.25\columnwidth]{final_images/aircraft/pegasus_2.jpg} &
    \includegraphics[width=0.25\columnwidth]{final_images/aircraft/yorkshire_2.jpg} &
    \includegraphics[width=0.25\columnwidth]{final_images/aircraft/wwii_1.jpg} & 
    \includegraphics[width=0.25\columnwidth]{final_images/aircraft/taken_3.jpg}
\end{tabular}
% \begin{tabular}{lll}
%     \multicolumn{3}{l} {\fontsize{11pt}{13pt}\textbf{Goal Class:} \texttt{ballplayer}}\\
%      \multicolumn{3}{l} {\fontsize{8pt}{10pt}\ttbfs{fiji players hormoncaine a picture of a mountain}}\\
%      \includegraphics[width=0.333\columnwidth]{final_images/ballplayer-append/fiji_players_hormoncaine_a_picture_of_a_mountain_2.jpg} &
%      \includegraphics[width=0.333\columnwidth]{final_images/ballplayer-append/fiji_players_hormoncaine_a_picture_of_a_mountain_3.jpg} &
%      \includegraphics[width=0.333\columnwidth]{final_images/ballplayer-append/fiji_players_hormoncaine_a_picture_of_a_mountain_4.jpg}
% \end{tabular}
% \newline
% \begin{tabular}{llll}
%     \ttbfs{fiji} & \ttbfs{players} & \ttbfs{hormon} & \ttbfs{caine} \\
%     \includegraphics[width=0.25\columnwidth]{final_images/ballplayer-append/fiji_1.jpg}&
%     \includegraphics[width=0.25\columnwidth]{final_images/ballplayer-append/players.jpg} &
%     \includegraphics[width=0.25\columnwidth]{final_images/ballplayer-append/hormon_5.jpg} & 
%     \includegraphics[width=0.25\columnwidth]{final_images/ballplayer-append/caine_3.jpg}
% \end{tabular}
\addtolength{\tabcolsep}{5.5pt} 
\caption{Task \ref{task: restricted prepending prompts 3} generated images with the class \texttt{aircraft}. Sample images generated using adversarial prompts. In both figures, the first row contains images generated by the optimized prompt and are classified by the ResNet18 classifier as the target class. 
The second row contains images generated from each individual token in the optimized prompt, none of which are classified as the target class. See Appendix \ref{app: additional examples} for more examples.}
\label{aircraft-and-ballplayer-prepend}
%\end{subfigure}
\vspace{-3ex}
\end{figure}
\subsubsection{Unrestricted Prompts}
\label{sec:manyimnet}

We consider a set of 400 target classes randomly selected from ImageNet classes that have a single token class name (e.g., excluding classes like \texttt{brown bear}). We report success rates for these 400 classes in \Cref{tab: results}. Both methods find prompts that are successful under both definitions from many target classes, with TuRBO consistently achieving a high rate of success. 

\paragraph{Higher-Level Classes.} In addition to the 400 regular ImageNet target classes, we randomly select a set of 150 higher-level classes from the ImageNet hierarchy. Higher-level ImageNet classes encompass some larger number of standard classes (i.e. \texttt{wolf} is a higher-level class encompassing the base-classes: \texttt{timber wolf}, \texttt{white wolf}, \texttt{red wolf}, \texttt{coyote}). For each higher-level class, the optimizer seeks a prompt that generates images that fall in any of the associated base-classes. The probability that an image falls in a higher-level class is the maximum over the probabilities of all associated base-classes. 

Success rates for the 150 higher-level classes are reported in \Cref{tab: results}. Optimizing for higher-level classes is more straightforward since the optimizer does not need to differentiate between highly related classes such as \texttt{timber wolf} and \texttt{white wolf}. We observe that success rates are therefore uniformly higher in this setting.

\subsubsection{Restricted Prompts}
\label{sec:restricted}

In \Cref{sec:manyimnet}, the optimization methods used an unconstrained vocabulary when designing prompts. Thus, when generating pictures of a wolf, the optimizers were allowed to use the token \texttt{wolf}, as well as other highly related words. In this section, we make this task significantly more challenging by forbidding the optimizers from using certain \textit{high-similarity tokens} in the output prompt.

We randomly select 12 target regular ImageNet classes and another 20 target higher-level ImageNet classes.
Since the restricted prompt optimization task is more difficult, we select these target classes from the subset of classes for which MPC success was achieved on the unrestricted task. 
The 12 selected regular ImageNet classes are listed in \Cref{tab:lower-classes-list}. The 20 selected higher-level ImageNet classes can be found in \Cref{tab:higher-classes-list}. 

We define a high-similarity token (HST) as a token $t$ where the prompt $p= t$ achieves low loss. We exclude all tokens which achieve a log probability of the target class higher than $-3.0$. In order to determine a comprehensive list of HSTs for each target class, we compute the loss for each of the 50k tokens available to the model. Precomputing the loss for these 50k tokens is computationally prohibitive-- thus we restrict our experiments to 32 target classes. We report results for optimization without access to HSTs for the 32 selected ImageNet classes in \Cref{tab: results}. Example optimal prompts with generated images can be found in \Cref{app: additional examples}. 
%



\subsubsection{Restricted Prepending Prompts}

We consider the prepending task introduced in Task \ref{task: restricted prepending prompts 3} of \Cref{sec: threat models} on a subset of the 32 classes used in \Cref{sec:restricted}. We prepend prompts onto the following three strings: \texttt{a picture of a dog}, \texttt{a picture of a mountain}, and \texttt{a picture of the ocean}. We provide quantitative results for all three variations of this task in \Cref{tab: results}. Because the prompts \CLS{} and \texttt{a picture of a \CLS{}} are no longer necessarily strong baselines when prepended to e.g. \texttt{a picture of a dog}, we no longer report OPB success for this task. Example adversarial prompts with generated images can be found in \Cref{aircraft-and-ballplayer-prepend}, with additional results in Appendix \ref{app: additional examples}. 
%
% \begin{figure}[t]
% \begin{center}
% \centerline{\includegraphics[width=0.48\textwidth]{plots/all_text_examples.pdf}}
% \caption{We provide examples of our models' optimized prompt in black, the original prompt to which we prepend in pink, and generated text in blue. (\textbf{Top Panel}) Example prompts that successfully reversed the sentiment of the generated text. (\textbf{Bottom Panel}) Example prompts that successfully generated text with a large number of target characters. }
% \label{text-examples}
% \end{center}
% \vskip -0.3in
% \end{figure}

% \begin{figure}
% \begin{center}
% \centerline{\includegraphics[width=0.48\textwidth]{plots/letters_plot.pdf}}
% \caption{ Average number of target characters generated by optimal prompts found by both optimizers as function of the total number of black-box function evaluations. Common letters are \texttt{a, e, i, f, t} and rare letters are \texttt{q, z, y}. Shaded regions around lines show standard error.}
% \label{letters-plot}
% \end{center}
% \vskip -0.4in
% \end{figure}
\subsection{Text Generation} 

%\vspace{-2ex}
% \begin{minipage}[c]{0.46\textwidth}
% \centering
% \includegraphics[width=0.9\textwidth]{plots/letters_plot.pdf}
% \captionof{figure}{Average number of target characters generated by optimal prompts found by both optimizers as function of the total number of black-box function evaluations. Common letters are \texttt{a, e, i, f, t} and rare letters are \texttt{q, z, y}. Shaded regions around lines show standard error.}
% \label{letters-plot}
% \end{minipage}
% \vspace{0.5cm}

With the rise in the use of generative text models, it's imperative to embed safety measures, ensuring their outputs align with human intentions while avoiding potential risks. We consider the relatively innocuous task of optimizing prompts for large language models to increase the perplexity of the output. Perplexity quantifies the overall level of likelihood of a sequence, measured by the negative log-likelihood as measured by a language model -- we use GPT-2 \citep{gpt2}. For a particular prompt, our objective is the average perplexity of the middle three of five generated outputs.

We use the Stable Vicuna 13B-v1.1 model \citep{vicuna2023}--a state of the art freely available LLM trained with human feedback--for text generation with a maximum generated length of $50$ tokens. We optimize perplexity with a maximum budget of 5,000 prompts, terminating early if no progress is made for 2,000 prompts in a row.

\begin{figure}[t]
    \centering
    % \includegraphics[width=0.8\columnwidth]{plots/perplexity_plot_standard_error.pdf}
    % trimming to estimate new figure size
    \includegraphics[width=\columnwidth]{final_images/perplexity_plot_standard_error.pdf}
    \caption{Plots of the maximum log perplexity with respect to the number of Vicuna 13B-v1.1 evaluations. The values are averaged over 20 random seeds, with the one standard error interval shaded. The full seed prompts are in \cref{tab: seed prompts}.}
    \label{fig: text perplexity plot}
    \vspace{-2ex}
\end{figure}
We optimize over prompts to prepend to a seed prompt (which we denote as `Meaning of Life', `Python', `SCAN', `Grammar'), and replicate these experiments 20 times per seed prompt. To choose seed prompts, we randomly selected prompts from the GPT4ALL and PromptSource datasets~\citep{gpt4all,bach2022promptsource} -- see \cref{tab: seed prompts} in \cref{app: text gen} for a list of all prompts. We use the Square Attack and TuRBO optimizers from \cref{sec: opt approaches} and also include a random search baseline, where we simply randomly sample tokens. We provide the performance of these approaches on four seed prompts in \cref{fig: text perplexity plot}, and more results in \cref{app: text gen}.


\cref{fig: text perplexity plot} demonstrates our ability to  increase the perplexity of the generated text, often by an order of magnitude. We also provide an example of the optimized adversarial prompt for the `Python' seed prompt in \cref{fig: text-examples}. This serves as a preliminary evidence that we may successfully optimize adversarial prompts to a desired criterion.





% \begin{figure}
%  \begin{subfigure}{.5\textwidth}
%         \centering
%     \begin{CJK*}{UTF8}{gbsn}
% \centering
% \begin{tabular}{p{7cm}}
% \textbf{Prompt: }\textcolor{red}{coordinate hip arts … filled via} \textcolor{darkgray}{Explain list comprehension in Python.}\\
% \textbf{Generated Examples: } \\

% 1. \textcolor{blue}{1. 单词:\textbackslash n 2. 词组: \textbackslash n 3. 短语：\textbackslash n \textbackslash n 关键词：\textbackslash n 1. 单词}\\
% %2. \textcolor{blue}{List comprehension in Python is a concise way to create a list from an existing iterable. It involves using a for loop and the ``extend" method to add items to a new list.}\\
% 2. \textcolor{blue}{1. Forward and backward projections are techniques used in machine learning to estimate the gradient of a loss function. 2. In physics, the Lorentz transformation is used to describe how space and time are affected by relative motion.}\\
% %4. \textcolor{blue}{Explain what? Can you please provide more context or clarify your question?}\\
% 3. \textcolor{blue}{I'd like to be called ``Alexa," as it is short, simple, and easy to remember. Plus, it has a nice ring to it!}
% \end{tabular}
% \caption{We provide five examples of our models' optimized prompt in red, the original prompt to which we prepend in gray, and generated text in blue.}
% \label{fig: text-examples}
% \end{CJK*}
%     \end{subfigure}
%      \begin{subfigure}{.5\textwidth}
%         \centering
%     \begin{CJK*}{UTF8}{gbsn}
% \centering
% \begin{tabular}{p{7cm}}
% \textbf{Prompt: }\textcolor{red}{coordinate hip arts … filled via} \textcolor{darkgray}{Explain list comprehension in Python.}\\
% \textbf{Generated Examples: } \\

% 1. \textcolor{blue}{1. 单词:\textbackslash n 2. 词组: \textbackslash n 3. 短语：\textbackslash n \textbackslash n 关键词：\textbackslash n 1. 单词}\\
% %2. \textcolor{blue}{List comprehension in Python is a concise way to create a list from an existing iterable. It involves using a for loop and the ``extend" method to add items to a new list.}\\
% 2. \textcolor{blue}{1. Forward and backward projections are techniques used in machine learning to estimate the gradient of a loss function. 2. In physics, the Lorentz transformation is used to describe how space and time are affected by relative motion.}\\
% %4. \textcolor{blue}{Explain what? Can you please provide more context or clarify your question?}\\
% 3. \textcolor{blue}{I'd like to be called ``Alexa," as it is short, simple, and easy to remember. Plus, it has a nice ring to it!}
% \end{tabular}
% \caption{We provide five examples of our models' optimized prompt in red, the original prompt to which we prepend in gray, and generated text in blue.}
% \label{fig: text-examples}
% \end{CJK*}
%     \end{subfigure}
%     \caption{Examples of more generated text}
% \end{figure}



==> icml_workshop/intro_workshop.tex <==
Foundation models (FMs) have demonstrated state-of-the-art performance across a diverse range of prediction and generation tasks. Large Language Models (LLMs), such as  GPT-3 \citep{gpt3}, PaLM \citep{palm}, and ChatGPT are capable of answering complex queries when given a short language prompt as instructions. In vision, FMs now come with an easy-to-use text interface that has revolutionized image generation. Text-To-Image Models (TTIM) such as DALL-E 2 \citep{dalle2}, Imagen \citep{imagen}, and Stable Diffusion \citep{StableDiff} are capable of generating a wide range of high-resolution images from text descriptions. 

The common thread amongst all these models is the use of a natural language prompt to influence the output of the model. By adjusting the words in a prompt, users can quickly and easily tweak the FM to generate text or images that better suit their task. This prompting interface has introduced a new mode of interaction with a model---instead of collecting datasets and fine-tuning models for a particular task, one simply changes words in a prompt. 

\begin{figure*}[!ht]
    \begin{subfigure}{.5\textwidth}
    
    \centering
    \begin{center}
\includegraphics[width=0.49\columnwidth]{final_images/final_mountain.jpg}
\includegraphics[width=0.49\columnwidth]{final_images/final_dog.jpg}
\caption{Images generated by Stable Diffusion v1.5 \citep{StableDiff} using the prompts \textbf{(Left)} `\texttt{a picture of a mountain}' and \textbf{(Right)} `\texttt{turbo lhaff\checkmark a picture of a mountain}', found by our method. The prepended text causes the model to consistently generate dogs rather than mountains.}
\label{first-page-img}
\end{center}
    \end{subfigure}
    \hspace{0.1cm}
    \begin{subfigure}{.5\textwidth}
        \centering
    \begin{CJK*}{UTF8}{gbsn}
\centering
 \tbox[\textbf{Prompt: }\textit{coordinate hip arts … filled via} Explain list comprehension in Python.]{
            \textbf{Generated Examples: } \\
            \begin{tabular}{l p{7cm}}
                 1. &  1. 单词:\textbackslash n 2. 词组: \textbackslash n 3. 短语：\textbackslash n \textbackslash n 关键词：\textbackslash n 1. 单词\\
                 2. & 1. Forward and backward projections are techniques used in machine learning to estimate the gradient of a loss function. \textbackslash 2. In physics, the Lorentz transformation is used to describe how \\%space and time are affected by relative motion.\\ 
                 3. & I'd like to be called ``Alexa," as it is short, simple, and easy to remember. Plus, it has a nice ring to it!
            \end{tabular}
        }
    \caption{Three examples of text generated from Vicuna 13B-v1.1 using our optimized prompt in italics and the original prompt to which we prepend. The generated text are nonsensical or irrelevant to the prompt.}
\label{fig: text-examples}
\end{CJK*}
    \end{subfigure}
    \caption{Examples of adversarial prompts and generated outputs.}
\vspace{-2ex}
\end{figure*}


% \begin{figure}[ht]
% \begin{center}
% \includegraphics[width=0.2\columnwidth]{plots/final_mountain.jpg}
% \hspace{1cm}
% \includegraphics[width=0.2\columnwidth]{plots/final_dog.jpg}
% \caption{Images generated by Stable Diffusion v1.5 \citep{StableDiff} using the prompts \textbf{(Left)} `\texttt{a picture of a mountain}' and \textbf{(Right)} `\texttt{turbo lhaff\checkmark a picture of a mountain}', found by our method. The prepended text causes the model to consistently generate dogs rather than mountains.}
% \label{first-page-img}
% \end{center}
% \vskip -0.2in
% \end{figure}
% \begin{figure}[ht]
% \begin{CJK*}{UTF8}{gbsn}
% \centering
% \begin{tabular}{l p{10cm}}
% \textbf{Prompt: }&\textcolor{red}{coordinate hip arts \u2026 filled via} \textcolor{black}{Explain list comprehension in Python.}\\
% \textbf{Generated Ex.: } &\\
% 1. &
%  \textcolor{blue}{1. 单词:\textbackslash n 2. 词组: \textbackslash n 3. 短语：\textbackslash n \textbackslash n 关键词：\textbackslash n 1. 单词}\\
% 2. &\textcolor{blue}{List comprehension in Python is a concise way to create a list from an existing iterable. It involves using a for loop and the ``extend" method to add items to a new list.}\\
% 3. &\textcolor{blue}{1. Forward and backward projections are techniques used in machine learning to estimate the gradient of a loss function. 
% 2. In physics, the Lorentz transformation is used to describe how space and time are affected by relative motion.}\\
% 4. & \textcolor{blue}{Explain what? Can you please provide more context or clarify your question?}\\
% 5. & \textcolor{blue}{I'd like to be called ``Alexa," as it is short, simple, and easy to remember. Plus, it has a nice ring to it!}
% \end{tabular}
% \caption{We provide five examples of our models' optimized prompt in red, the original prompt to which we prepend in black, and generated text in blue.}
% \label{fig: text-examples}
% \end{CJK*}
% \end{figure}
However, it is becoming apparent that small variations in the prompt can lead to substantial differences in the model output. For example, prompting is known to be sensitive to the order of sentences \cite{lu2021fantastically}, variations in the template \cite{jiang2020can}, and the specific examples provided in the prompt \cite{liu2021makes}. Certain prompts can also result in strange or unusual behavior. For example, gibberish words from generated images such as ``Apoploe vesrreaitais'' can be used as a prompt to generate animals such as birds \cite{daras2022discovering}. 

Recent work has seen researchers crafting adversarial prompts that exploit these vulnerabilities to extract information or induce malevolent behaviors. For example, \citet{perez2022ignore} designed adversarial prompts that induce specific behaviors in an LLM, such as repeating its original prompt or outputting a particular string. \citet{xu2022exploring} studied backdoors and adversarial triggers for LLMs fine-tuned on target tasks. However, these latter adversarial attacks require gradient information and the ability to modify the weights of the LLM. Such attacks are not possible on closed-source, general purpose FMs such as ChatGPT or DALL-E 2 that are used for a wide variety of unstructured tasks. \emph{How do we craft adversarial prompts for general tasks on foundation models with only query access?}

\paragraph{Our Contributions.}
In this paper, we develop a framework for finding adversarial prompts in the black-box setting for general language and vision objectives. We focus specifically on \emph{black-box} attacks as many foundation models are not publicly available, e.g. ChatGPT and DALL-E 2 only have API access. We build upon tools for black-box adversarial attacks traditionally used in the vision setting but instead leverage these tools to search for adversarial prompts. The main challenges are the high dimensionality and discrete nature of the token space. These properties drastically increase the sample complexity and slow down the convergence of classic black-box adversarial attacks. To address these issues, we develop a Token Space Projection (TSP) to map a continuous, lower-dimensional embedding space to the set of discrete language tokens. Our projected variations of black box attacks are capable of finding adversarial prompts, which we demonstrate across a range of vision and language tasks. Our main contributions are:

\begin{CompactEnumerate}
    \item We develop a framework for finding adversarial prompts using a Token Space Projection operator. This operator bridges the continuous word embedding space with the discrete token space, and enables the use of black-box attacks to find adversarial prompts. 
    \item We demonstrate how our framework can automatically find standalone or prepended prompts that cause text-to-image models to output specific image classes. We can further find adversarial prompts that exclude tokens related to the target class. 
    \item Our framework can also find adversarial prompts that alter text generation. For example, we find adversarial prompts that generate irrelevant or incoherent text, or text in different languages.
\end{CompactEnumerate}


==> icml_workshop/results_table_workshop.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table}[]
\caption{Success rates for TuRBO and Square Attack for all image generation tasks. We report the proportion of these classes for which each method achieved success according to our two measures of success discussed in \Cref{sec:success-methods}, with `Both` referring to MPC and OPB. Single refers to single/regular image-net classes. Higher refers to image-net classes further up in the image-net class hierarchy.}
\centering
\begin{tabular}{l l r r r r}
\toprule
Task                                                                             & \multicolumn{1}{l }{Metric} & \begin{tabular}[c]{@{}c@{}}TuRBO\\ (Single)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Square\\ (Single)\end{tabular} & \begin{tabular}[c]{@{}c@{}}TuRBO\\ (Higher)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Square\\ (Higher)\end{tabular} \\ 
\midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Task 1\end{tabular}} & MPC                        & 18.5\%                                                   & 1.5\%                                                     & 42.0\%                                                   & 12.7\%                                                    \\
                                                                                 & OPB                        & 36.8\%                                                   & 13.5\%                                                    & 61.3\%                                                   & 23.3\%                                                    \\
                                                                                 &  Both             & 10.5\%                                                   & 0.0\%                                                     & 36.0\%                                                   & 7.3\%                                                     \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Task 2\end{tabular}}   & MPC                        & 58.3\%                                                   & 8.3\%                                                     & 60.0\%                                                   & 0.0\%                                                     \\
                                                                                 & OPB                        & 83.3\%                                                   & 58.3\%                                                    & 75.0\%                                                   & 70.0\%                                                    \\
                                                                                 & Both                    & 50.0\%                                                   & 8.3\%                                                     & 55.0\%                                                   & 10.0\%                                                    \\ \midrule
\begin{tabular}[c]{@{}c@{}}Task 3\end{tabular}           & MPC                        & 25.0\%                                                   & 0.0\%                                                     & 37.3\%                                                   & 0.0\%           \\\bottomrule  \\
\end{tabular}

\label{tab: results}
\vspace{-5ex}
\end{table}
% \begin{table*}[!ht]
% \begin{small}
%     \begin{center}
% \caption{Success rates for TuRBO and Square Attack for all image generation tasks. We report the proportion of these classes for which each method achieved success according to our two measures of success discussed in \Cref{sec:success-methods}. Single refers to single/regular image-net classes. Higher refers image-net classes further up in the image-net class hierarchy (classes that encompass multiple single sub-classes).}
%     \label{tab: results}
% \renewcommand{\arraystretch}{1.6}
% \setlength\tabcolsep{12pt}
%     \centering
%     \begin{tabular}{ccl  r r}
% \toprule     
%       \multicolumn{2}{c}{Task} & Metric   &  TuRBO  & Square Attack \\
% \cmidrule(r){1-5}
% \multirow{6}{*}{\rotatebox[origin=c]{0}{ {\textit{Task \ref{task: unrestricted prompts 1} Unrestricted}}}}  &\multirow{3}{*}{\rotatebox[origin=c]{0}{Single}} & MPC   & 18.5\% & 1.5\% \\
%  &  &  OPB   & 36.8\% & 13.5\% \\
%  &  &  MPC and OPB   & 10.5\% & 0.0\% \\
% \cline{2-5}
% &\multirow{3}{*}{\rotatebox[origin=c]{0}{Higher}} & MPC   & 42.0\% & 12.7\%  \\
%  &  &  OPB   & 61.3\% & 23.3\%   \\
%  &  &  MPC and OPB   & 36.0\% & 7.3\% \\
%  \hline \hline
% \multirow{6}{*}{\rotatebox[origin=c]{0}{ {\textit{Task \ref{task: restricted prompts 2} Restricted}}}}  &\multirow{3}{*}{\rotatebox[origin=c]{0}{Single}} & MPC   & 58.3\% & 8.3\%  \\
%  &  &  OPB   & 83.3\% & 58.3\%  \\
%  &  &  MPC and OPB   & 50.0\% & 8.3\%  \\
% \cline{2-5}
% &\multirow{3}{*}{\rotatebox[origin=c]{0}{Higher}} & MPC   & 60.0\% &  0.0\% \\
%  &  &  OPB   & 75.0\% & 70.0\%  \\
%  &  &  MPC and OPB   & 55.0\% & 10.0\% \\
% \hline \hline
% \multirow{2}{*}{\rotatebox[origin=c]{0}{ {
% \parbox{2.5cm}{
% \centering
% \textit{
% Task \ref{task: restricted prepending prompts 3} Restricted}\\ \textit{Prepending}}
% }
% }
% }
% & Single & MPC   & 25.0\% & 0.0\%
% \\
% \cline{2-5}
% &Higher  & MPC   & 37.3\% & 0.0\% \\
% \bottomrule

% \end{tabular}
% \end{center}
% \end{small}
% \end{table*}

